Paramater Optimization for Manipulator Motion Planning using a Novel Benchmark Set

Sampling-based motion planning algorithms have been continuously developed for more than two decades. Apart from mobile robots, they are also widely used in manipulator motion planning. Hence, these methods play a key role in collaborative and shared workspaces. Despite numerous improvements, their performance can highly vary depending on the chosen parameter setting. The optimal parameters depend on numerous factors such as the start state, the goal state and the complexity of the environment. Practitioners usually choose these values using their experience and tedious trial and error experiments. To address this problem, recent works combine hyperparameter optimization methods with motion planning. They show that tuning the planner's parameters can lead to shorter planning times and lower costs. It is not clear, however, how well such approaches generalize to a diverse set of planning problems that include narrow passages as well as barely cluttered environments. In this work, we analyze optimized planner settings for a large set of diverse planning problems. We then provide insights into the connection between the characteristics of the planning problem and the optimal parameters. As a result, we provide a list of recommended parameters for various use-cases. Our experiments are based on a novel motion planning benchmark for manipulators which we provide at https://mytuc.org/rybj.

==> related_work.tex <==
\section{Related Work}

In recent years, several approaches have addressed the problem of hyperparameter tuning in \gls{sbmp} for manipulators. In \cite{BurgerAutomated}, the authors utilize a random forest model to tune parameters of several algorithms provided in the \gls{ompl} \cite{sucan2012ompl}. The authors achieved reduced planning times and costs in a few pre-defined pick-and-place scenarios.
Cano et al. investigated several optimization methods while considering the BKPIECE \cite{bkpiece} and RRT-Connect \cite{rrtconnect} algorithm implemented in \gls{ompl}. Using a tabletop reaching scenario, the authors show that planning time can be reduced by a factor of 4.5. In addition, randomized planning problems are used to show that the tuned parameters generalize well across various setups.
Moll et al. use \gls{bohb} \cite{BOBHFalkner} optimize over an extensive search space that includes several planning algorithms and their parameters. Hence, the authors manage to find the best performing approach together with its tuned parameters. For evaluation, the authors use several classes of planning problems such as reaching into a shelf or into a box. The considered optimization criteria are planning and execution speed.
In the same work the authors also demonstrate that optimizing on a small set of problem classes can lead to good performance in all of them. However, it was not shown to which number of classes and to which variety in complexity this holds.
Furthermore, none of the mentioned works utilize a parallelized planner. It is thus not clear to which extent parameter optimization can improve the results in such a setup.
